Gammapy - A prototype for the CTA science tools

Gammapy is a Python package for high-level gamma-ray data analysis built on Numpy, Scipy and Astropy. It enables us to analyze gamma-ray data and to create sky images, spectra and lightcurves, from event lists and instrument response information, and to determine the position, morphology and spectra of gamma-ray sources. So far Gammapy has mostly been used to analyze data from H.E.S.S. and Fermi-LAT, and is now being used for the simulation and analysis of observations from the Cherenkov Telescope Array (CTA). We have proposed Gammapy as a prototype for the CTA science tools. This contribution gives an overview of the Gammapy package and project and shows an analysis application example with simulated CTA data.

==> Makefile <==
TARGET=gammapy-icrc2017
LATEX=pdflatex
BIBTEX=bibtex

all: $(TARGET).pdf

$(TARGET).pdf: *.tex $(TARGET).bib

%.pdf: %.tex
	$(LATEX) $<
	$(BIBTEX) $*
	$(LATEX) $<
	$(LATEX) $<

make clean:
	- rm -f $(TARGET).pdf $(TARGET).aux $(TARGET).log $(TARGET).bbl $(TARGET).blg *.aux $(TARGET).tar.gz

# Tarball for ArXiv submission
tarball:
	- tar -cvzf $(TARGET).tar.gz \
	$(TARGET).tex \
	$(TARGET).bib \
	$(TARGET).bbl \
	figures/gammapy-stack.pdf \
	figures/gammapy_example_sky_image.png \
	examples/code_events_image.pdf \
	PoSlogo.pdf \
	JHEP.bst \
	PoS.cls \
	Makefile \

